Edge-aware Bidirectional Diffusion for Dense Depth Estimation from Light Fields

We present an algorithm to estimate fast and accurate depth maps from light fields via a sparse set of depth edges and gradients. Our proposed approach is based around the idea that true depth edges are more sensitive than texture edges to local constraints, and so they can be reliably disambiguated through a bidirectional diffusion process. First, we use epipolar-plane images to estimate sub-pixel disparity at a sparse set of pixels. To find sparse points efficiently, we propose an entropy-based refinement approach to a line estimate from a limited set of oriented filter banks. Next, to estimate the diffusion direction away from sparse points, we optimize constraints at these points via our bidirectional diffusion method. This resolves the ambiguity of which surface the edge belongs to and reliably separates depth from texture edges, allowing us to diffuse the sparse set in a depth-edge and occlusion-aware manner to obtain accurate dense depth maps.

==> src-figures/patches.tex <==

\begin{figure}[tp]
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{./Figures/patches/oriented-patches-a.png}
\end{subfigure} 

\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{./Figures/patches/oriented-patches-b.png}
\end{subfigure} %
\vspace{-0.25cm}
\caption{When performing a plane sweep, selecting patches centered around a point $p \in O$ leads to incorrect depth estimates as all points $p$ in our algorithm lie near edges. If this edge is an occlusion edge, we get misleading cost estimates. This is seen in the top row, where even though the patch in (\textit{\textbf{a}}) is being projected at the ground truth depth $d_{GT}$ in (\textit{\textbf{b}}), the cost volume still has high variance (\textbf{\textit{c}}). We propose using one-sided, oriented patches around $p$ instead. As show in the bottom row, doing so creates a volume with much lower variance, allowing us to correctly identify $d_{GT}$ as the correct depth.} 
\label{fig:oriented-patches}
\end{figure}

==> src-figures/results-error.tex <==

\begin{figure*}[t!]
\centering
\includegraphics[width=0.75\textwidth]{./Figures/error.pdf}
\caption{A visualization of the absolute disparity error. Our method has less pixels with very high error. This can be seen in the fewer regions of red for our method compared to the baselines.} 
\label{fig:results-error}
\end{figure*}

==> src-figures/results-hci.tex <==

\begin{figure*}[tp]
\centering
\includegraphics[width=\textwidth]{./Figures/results-hci.pdf}
\vspace{-0.25cm}
\caption{Results on the synthetic light fields of the HCI dataset. \emph{Left to right:} Jeon et al.~\cite{jeon2015}, Zhang et al~\cite{zhang2016}, Jiang et al.~\cite{jiang2018}, Shi et al.~\cite{shi2019}, our method, and finally, the ground truth. } 
\label{fig:results-hci}
\end{figure*}

==> src-figures/results-lego.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/lego.png}
\end{subfigure}%
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/lego-zhang.png}
\end{subfigure}%
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/lego-jeon.png}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/lego-jiang.png}
\end{subfigure}%
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/lego-shi.png}
\end{subfigure}%
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/lego-ours.png}
\end{subfigure}
\caption{\emph{Lego} real-world light field scene. In western order: central light field view, non-learning-based depth map estimation methods of Jeon et al.~\cite{jeon2015} and Zhang et al.~\cite{zhang2016}, learning-based methods of Jiang et al.~\cite{jiang2018} and Shi et al.~\cite{shi2019}, and finally our non-learning-based method. Our method produces more accurate results than the compared non-learning-based methods and the learning-based method of Jiang et al.~\cite{jiang2018}, while being significantly faster to compute (13--20$\times$). Compared to the learning-based method of Shi et al.~\cite{shi2019}, we have comparable average error and runtime.} 
\label{fig:results-lego}
\end{figure*}

==> src-figures/results-stanford.tex <==
\begin{figure*}
\centering
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/results-bunny.png}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/results-bulldozer.png}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/results-chess.png}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/results-eucalyptus.png}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/results-jelly-beans.png}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/results-jewels.png}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/results-lego.png}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/results-tarot.png}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{./Figures/results/results-truck.png}
\end{subfigure}
\vspace{-0.25cm}
\caption{Stanford lightfield scenes. From left to right: central view, non-learning-based estimations of Jeon et al.~\cite{jeon2015} and Zhang et al.~\cite{zhang2016}, learning-based methods of Jiang et al.~\cite{jiang2018} and Shi et al.~\cite{shi2019}, and our non-learning-based method.} 
\label{fig:results-stanford}
\end{figure*}

==> src/4a.experiments-non-learning.tex <==

\newcolumntype{x}[1]{%
>{\centering\hspace{0pt}}p{#1}}%

\setlength{\tabcolsep}{1.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t]
\begin{center}
\caption{Quantitative comparison of our method with two baseline non-learning-based methods on the central view of four 9 $\times$ 9 synthetic light fields. The running time shown is the cost to estimate depth for a single view of the light field. `BP($x$)' is the number of \emph{bad pixels} above threshold $x$ in error. Our approach has less error than competing methods while being $\sim$8-11$\times$ faster.}
\vspace{1mm}
\label{table:non-learning-based-comparison}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|x{1.8em}|x{1.6em}|x{2.12em}|x{1.8em}|x{2.2em}|x{2.12em}|x{2.2em}|x{1.8em}|x{2.12em}|x{2.2em}|x{2.2em}|x{2.12em}|x{1.8em}|x{2.2em}|c}
\hline
\multirow{2}{4em}{Light Field} & \multicolumn{3}{c}{Run time (s)} & \multicolumn{3}{c}{MSE $\times$ 100} & \multicolumn{3}{c}{BP(0.01)} & \multicolumn{3}{c}{BP(0.03)} & \multicolumn{3}{c}{BP(0.07)} \\
\cline{2-16}
& \cite{jeon2015} & \cite{zhang2016} & \small{Ours} & \cite{jeon2015} & \cite{zhang2016} & \small{Ours} & \cite{jeon2015} & \cite{zhang2016} & Ours & \cite{jeon2015} & \cite{zhang2016} & Ours & \cite{jeon2015} & \cite{zhang2016} & Ours\\
\hline
\textit{Sideboard} & 754 & 537 & \textbf{62.1} & 3.21 & 1.02 & \textbf{0.89} & \textbf{63.7} & 78.0 & 73.8 & 40.6 & 42.0 & \textbf{37.4} & 26.7 & \textbf{14.4} & 16.2\\

\textit{Dino} & 805 & 531 & \textbf{62.4} & 1.73 & \textbf{0.36} & 0.45 & 76.4 & 77.3 & \textbf{69.4} & 48.6 & 40.4 & \textbf{30.8} & 22.7 & \textbf{6.90} & 10.4\\

\textit{Cotton} & 748 & 530 & \textbf{59.4} & 12.5 & 1.81 & \textbf{0.68} & \textbf{52.6} & 75.3 & 56.2 & 21.4 & 34.7 & \textbf{18.0} & 9.05 & \textbf{4.40} & 4.90\\

\textit{Boxes} & 736 & 541 & \textbf{58.5} & 16.0 & 7.90 & \textbf{6.70} & \textbf{69.3} & 84.7 & 76.8 & \textbf{45.5} & 55.3 & 47.9 & 26.8 & \textbf{18.9} & 28.3\\
\hline

\textit{\textbf{Average}} & 761 & 535 & \textbf{60.6} & 8.37 & 2.77 & \textbf{2.18} & \textbf{65.5} & 78.8 & 69.0 & 39.1 & 40.2 & \textbf{33.5} & 21.3 & \textbf{11.2} & 14.9\\
\hline
\end{tabular}
}
\end{center}
\end{table*}
\setlength{\tabcolsep}{1.4pt}


==> src/4b.experiments-learning.tex <==

\setlength{\tabcolsep}{0.9pt}
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t]
\begin{center}
\caption{\nk{Merge table 1 and 2}.  Quantitative comparison of our method with two baseline learning-based methods on the central view of a set of four 9 $\times$ 9 synthetic light fields. The running time shown is the cost to estimate depth for a single view of the light field. `BP($x$)' is the number of \emph{bad pixels} which fall above threshold $x$ in error. Our approach has lower error than the method of Jiang et al.~\cite{jiang2018} and $\sim$8$\times$ faster runtime; our method has competitive error to the state of the art method of Shi et al.~\cite{shi2019}, without requiring any learning. As baseline methods have higher MSE but fewer bad pixels, the errors they do have must be larger. We confirm this by visualizing error plots in Figure~\ref{fig:results-error}}.
\vspace{1mm}
\label{table:learning-based-comparison}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|x{2.1em}|x{1.8em}|x{2.12em}|x{2.2em}|x{1.8em}|x{2.12em}|x{1.8em}|x{2.2em}|x{2.12em}|x{1.8em}|x{2.2em}|x{2.12em}|x{2.2em}|x{2.2em}|c}
\hline
\multirow{2}{4em}{Light Field} & \multicolumn{3}{c}{Run time (s)} & \multicolumn{3}{c}{MSE * 100} & \multicolumn{3}{c}{BP(0.01)} & \multicolumn{3}{c}{BP(0.03)} & \multicolumn{3}{c}{BP(0.07)}\\
\cline{2-16}
& \cite{shi2019} & \cite{jiang2018} & Ours & \cite{shi2019} & \cite{jiang2018} & Ours & \cite{shi2019} & \cite{jiang2018} & Ours & \cite{shi2019} & \cite{jiang2018} & Ours & \cite{shi2019} & \cite{jiang2018} & Ours\\
\hline
\textit{Sideboard} & 72.3 & 507 & \textbf{62.1} & 1.12 & 1.96 & \textbf{0.89} & 53.0 & \textbf{47.4} & 73.8 & 20.4 & \textbf{18.3} & 37.4 & \textbf{2.70} & 9.30 & 16.2 \\
\textit{Dino} & \textbf{59.3} & 500 & 62.4 & \textbf{0.43} & 0.47 & 0.45 & 43.0 & \textbf{29.8} & 69.4 & 13.1 & \textbf{8.80} & 30.8 & 4.31 & \textbf{3.60} & 10.4\\
\textit{Cotton} & 79.8 & 500 & \textbf{59.4} & 0.88 & 0.97 & \textbf{0.68} & 38.8 & \textbf{25.4} & 56.2 & 9.60 & \textbf{6.30} & 18.0 & 2.80 & \textbf{2.00} & 4.9\\
\textit{Boxes} & \textbf{56.2} & 491 & 58.5 & 8.48 & 11.6 & \textbf{6.70} & 66.5 & \textbf{51.8} & 76.8 & 37.1 & \textbf{27.0} & 47.9 & 21.9 & \textbf{18.3} & 28.3\\
\hline
\textit{\textbf{Average}} & 66.9 & 500 & \textbf{60.6} & 2.72 & 3.75 & \textbf{2.18} & 50.3 & \textbf{38.6}  & 69.0 & 20.1 & \textbf{15.1} & 33.5 & \textbf{7.92} & 8.30 & 14.9 \\
\hline
\end{tabular}
}
\end{center}
\end{table*}
\setlength{\tabcolsep}{1.4pt}


==> src/4c.experiments-realworld.tex <==
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.2}
\begin{table}[t]
\begin{center}
\caption{The average reprojection error onto the four corner views. We show results for real world light fields from the EPFL (top) and Stanford datasets (bottom). The error for each view is computed as the mean of the absolute difference between the real and reprojected view times $10^{-2}$. Our method performs consistently better than all baselines on the EPFL dataset.}
\label{table:reprojection-error}
\vspace{1mm}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|x{3em}x{3em}x{3em}x{3em}c}
\hline
\multirow{2}{4em}{Light Field} & \multicolumn{5}{c}{Reprojection Error} \\
\cline{2-6}
& \cite{shi2019} & \cite{jiang2018} & \cite{zhang2016} & \cite{jeon2015} & Ours\\
\hline
\textit{Bikes} & 5.2 & 5.3 & 5.3 & 5.2 & \textbf{2.5} \\
\textit{Grid} & 6.9 & 6.8 & 6.6 & 6.6 & \textbf{4.5} \\
\textit{Silos} & 3.3 & 4.2 & 2.5 & 3.5 & \textbf{2.3} \\
\textit{Sphynx} & 5.4 & 5.8 & 5.6 & 5.7 & \textbf{2.6} \\
\hline
\textit{\textbf{Average}} & 5.2 & 5.5 & 5.0 & 5.3 & \textbf{3.0} \\
\hline
\textit{Bunny}  & 1.2 & 1.6 & 1.3 & 2.1 & \textbf{1.1} \\
\textit{Bulldozer} & \textbf{2.0} & 3.4 & 2.1 & 8.9 & 2.4 \\
\textit{Chess}  & \textbf{1.7} & \textbf{1.7} & \textbf{1.7} & 6.6 & 1.8\\
\textit{Eucalyptus}   & 1.2 & 1.6 & 1.3 & 3.5 & \textbf{1.1}\\
\textit{Jelly-Beans} & 1.5 & 1.7 & \textbf{1.4} & 3.3 & 1.7 \\
\textit{Jewels} & \textbf{2.3} & 2.5 & 2.7 & 6.6 & \textbf{2.3} \\
\textit{Lego} & \textbf{2.5} & 4.4 & 3.1 & 7.6 & 3.0 \\
\textit{Tarot} & \textbf{9.9} & 17 & 15 & 20 & 17 \\
\textit{Truck} & \textbf{1.4} & 4.9 & 1.7 & 4.1 & \textbf{1.4} \\
\hline
\textit{\textbf{Average}} & \textbf{2.6} & 4.3 & 3.4 & 7.0 & 3.6 \\
\hline
\end{tabular}
}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}





%& & Bunny & Bulldozer & Chess & Eucalyptus & Jelly-Beans & Jewels & Lego & Tarot & Truck & Average & Bikes & Grid & Silos & Sphynx & Average

%\hline
%\cite{shi2019} & 1.2 & 2.0 & 1.7 & 1.2 & 1.5 & 2.3 & 2.5 & 9.9 & 1.4 & 2.6 & 5.1 & 6.89 & 3.3 & 5.4 & X \\
%& \cite{jiang2018} & 1.6 & 3.4 & 1.7 & 1.6 & 1.7 & 2.5 & 4.4 & 17 & 4.9 & 4.3 & 5.3 & 6.8 & 4.2 & 5.8 & X \\
%\cite{zhang2016} & 1.3 & 2.1 & 1.7 & 1.3 & 1.4 & 2.7 & 3.1 & 15 & 1.7 & 3.4 & 5.2 & 6.6 & 4.0 & 5.7 & X \
%\cite{jeon2015} & 2.1 & 8.9 & 6.6 & 3.5 & 3.3 & 6.6 & 7.6 & 20 & 4.1 & 7.0 & 5.2 & 6.6 & 3.5 & 5.7 & X\\
%\cite{zhang2016} & 1.2 & 2.6 & 1.7 & 1.2 & 1.8 & 2.3 & 3.1 & 18 & 1.5 & 3.7 & 5.3 & 6.6 & 3.5 & 5.6 & X\\

%\textit{Bikes}  & \textbf{5.12} & 5.33 & \textbf{5.24} & 5.22 & 5.25 \\
%\textit{Sphynx} & \textbf{5.40} & 5.76 & 5.71 & 5.69 & \textbf{5.63} \\
%\textit{Silos}  & \textbf{3.25} & 4.16 & 4.07 & \textbf{3.45} & 3.50\\
%\textit{Grid}   & 6.89 & \textbf{6.84} & \textbf{6.58} & 6.63 & 6.63\\
%\textit{Lego} & \textbf{2.57} & 14.3 & 3.12 & 16.4 & \textbf{3.10} \\7
%\hline
%\textit{\textbf{Average}} & \textbf{4.65} & 7.27 & 4.94 & 7.47 & \textbf{4.82} \\



==> src/4d-yucer-comparison.tex <==
\newcolumntype{x}[1]{%
>{\centering\hspace{0pt}}p{#1}}%

\setlength{\tabcolsep}{1.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t]
\begin{center}
\caption{Evaluating the key steps of sparse depth labeling (Section~\ref{sec:method-sparse-labels}) and diffusion direction estimation (Section~\ref{sec:dense-propagation}) in our approach by replacing them with the algorithms of Khan et al.~\cite{khan2019} and Yucer et al.~\cite{yucer2016} respectively. The `bad pixels' metric $\mathrm{BP}(x)$ measures the percentage of pixels with an absolute error higher than threshold $x$. The best results are highlighted in \gold{gold}. Our approach to the key steps provides consistently lower error. }
\vspace{1mm}
\label{table:yucer-comparison}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|x{3em}|x{3em}|x{3em}|x{3em}|x{3em}|x{3em}|x{3em}|x{3em}|x{3em}|x{3em}|x{3em}|r}
\hline
\multirow{2}{4em}{Light Field}  & \multicolumn{3}{c}{MSE $\times$ 100} & \multicolumn{3}{c}{BP(0.01)} & \multicolumn{3}{c}{BP(0.03)} & \multicolumn{3}{c}{BP(0.07)} \\
\cline{2-13}
& \cite{khan2019} & \cite{yucer2016} & Ours & \cite{khan2019} & \cite{yucer2016} & Ours & \cite{khan2019} & \cite{yucer2016} & Ours & \cite{khan2019} & \cite{yucer2016} & Ours\\
\hline
\textit{Sideboard}  & 7.48 & 1.26 & \gold{1.03} & 96.5 & \gold{73.4} & 79.1 & 89.5 & \gold{45.2} & 46.0 & 74.7 & 21.4 & \gold{17.6}\\

\textit{Dino} & 6.77 & 1.26 & \gold{0.45} & 96.9 & \gold{67.7} & 70.9 & 90.5 & 46.1 & \gold{31.4} & 78.0 & 28.0 & \gold{\phantom{0}9.4}\\

\textit{Cotton} & 10.7 & 1.81 & \gold{0.70} & 97.9 & 76.2 & \gold{67.4} & 93.9 & 46.1 & \gold{27.0} & 82.9 & 24.4 & \gold{\phantom{0}5.8}\\ % Phantom makes the gold box full width

\textit{Boxes}  & 16.1 & 11.9 & \gold{7.52} & 97.2 & 85.5 & \gold{82.0} & 91.2 & 68.1 & \gold{51.8} & 78.9 & 30.7 & \gold{24.4}\\
\hline

\textit{\textbf{Average}} & 10.3 & 4.06 & \gold{2.43} & 97.1 & 75.7 & \gold{74.8} & 91.3 & 51.4 & \gold{39.1} & 78.9 & 30.7 & \gold{14.3}\\
\hline
\end{tabular}
}
\end{center}
\end{table*}
\setlength{\tabcolsep}{1.4pt}

